Preventing Denial of Service Attacks in IoT Networks through Verifiable Delay Functions

Permissionless distributed ledgers provide a promising approach to deal with the Internet of Things (IoT) paradigm. Since IoT devices mostly generate data transactions and micropayments, distributed ledgers that use fees to regulate the network access are not an optimal choice. In this paper, we study a feeless architecture developed by IOTA and designed specifically for the IoT. Due to the lack of fees, malicious nodes can exploit this feature to generate an unbounded number of transactions and perform a denial of service attacks. We propose to mitigate these attacks through verifiable delay functions. These functions, which are non-parallelizable, hard to compute, and easy to verify, have been formulated only recently. In our work, we design a denial of service prevention mechanism which addresses network heterogeneity, limited node computational capabilities, and hardware-specific implementation optimizations. Verifiable delay functions have mostly been studied from a theoretical point of view, but little has been done in tangible applications. Hence, this paper can be considered as a pioneer work in the field, since it builds a bridge between this theoretical mathematical framework and a real-world problem.

==> discussion.tex <==
\section{Discussion}\label{sec:discussion}

\subsection{Node accountability and Sybil protection}\label{sec:sybil}
Node accountability is a fundamental required component to enable our proposed VDF-based anti spam mechanism. To this end, we envision using common public key cryptography to sign certain data and to link it to its issuing node in a tamper proof way. Additionally, we require that the issuing node adds its public key to every signed message. This way, every node can verify the authenticity of the issuing node without the need for some form of global database of IDs and keys. It is important to note that these mechanisms only need to be implemented to protect the communication layer and that keys, IDs and signatures do not need to be stored in the Tangle once processed by the node.

When node identities are relevant, a distributed system becomes vulnerable to Sybil attacks~\cite{Douceur2002}, where a malicious entity masquerades as multiple counterfeit identities. This would overcome any mechanism that relies on a limited number of such identities and would open the network to coordinated attacks. One very common way to make such a Sybil attack harder is the so-called resource testing, where each identity has to prove the ownership of certain difficult-to-obtain resources. Since in the cryptocurrency world users own a certain amount of tokens, we propose a reputation system based on the ownership of such tokens (see definitions in Section~\ref{sec:model}). The details of the reputation system are out of the scope of this paper.

Instead, here we want to suggest how to link the difficulty parameter $\tau$ (hence, throughput $\gamma$) to the reputation value. An important requirement is that reputation and throughput are \textit{linearly} proportional: on the one hand, a sublinear proportionality would incentivize nodes to split, violating the Sybil protection purpose; on the other hand, superlinearity would motivate nodes to pool together. According to this discussion, a node sets the difficulty $\tau$ as
\begin{equation*}
    \gamma(\tau) = \alpha \cdot m_i,
\end{equation*}
where $\alpha$ is a scale parameter. The function between the throughput and the difficulty $\tau$ can be easily inferred empirically as we have shown in Figure~\ref{fig:eval_cpp}.

\subsection{RSA key length}\label{sec:rsa_length}
The core of the security lies in the RSA private key secret. As soon as an attacker guesses the private key he can run VDFs evaluations in a very short time. The longer the private key, the more secure our protocol is. Using large keys implies more CPU time spent, more battery consumption and larger network overhead but yields a better security. It is then important to chose a convenient RSA key length when we deal with tiny devices. One way of evaluating the security of a RSA key length is to use the equivalency table between RSA keys-length and the bit level security in Table \ref{tab:rsa_length}.\cite{Martin2008} A bit-level security of $K$ bits means it takes $2^K$ computations to brute force the solution. It is also equivalent to the security of a block cipher algorithm using keys of size $K$ \cite{Albermany}.

\begin{table}[ht]
    \centering
    \begin{tabular}{c|c}
    RSA key length & Bit-level security\\
    \hline
    1024 & 80\\
    2048 & 112\\
    3072 & 128\\
    7,168 & 192\\
    15,360 & 256\\
    \end{tabular}
    \caption{Equivalency between RSA keys length and bit-level security}
    \label{tab:rsa_length}
\end{table}

The main RSA factorization \cite{Brent} attack are, in increasing order of performance, the Lenstra Elliptic-Curve algorithm \cite{Dixon}, efficient especially for small prime factors, the Quadratic Sieve (QS) algorithm \cite{Pomerance}, efficient for numbers under 100 bits and the General Number Field Sieve~\cite{Lenstra1993}, more complex than the QS but the most efficient algorithm for numbers above 100 bits.

It is then interesting to consider the cost of such an attack. We follow a similar estimation as Cybernetica in 2015 \cite{Cybernetica2016}. Renting a \texttt{c5.metal} AWS server for 3 years grants you access to a 3.6 Ghz machine with 96 cores for \$40,000. It then yields around $2^{64,8}$ instructions in 3 years. Then breaking a 1024 bits RSA key would cost around 1.5 billion USD. For a 2048 bits key it would cost \$$5\cdot10^{18}$. However it has to be nuanced because Cybernetica claimed in 2016 that factoring cost a 1024 RSA key could be reduced \$1 million \cite{Cybernetica2016}. When it comes to hijack a cryptocurrency, one million dollars is an amount a big organization can invest. Finally, the US agency for standardization of cryptographic functions, the NIST, reports that 112 bit-level algorithms should not be used beyond 2030 and we should then use 128+ bit-level algorithms. We then believe using a 1024 bits RSA is too weak and we should consider using 2048 bits keys with a periodical modulus refresh. Using 1024 bits RSA keys can be considered but should be refreshed very often to discourage attackers to factorize it.

\subsection{Improving the proof computation}\label{sec:proof_improve}
The proof part of the VDF takes roughly the same time as the evaluation but can be computed in the same time because it depends on the evaluation result. Increasing performances in this part of the protocol is of a great importance. We will only give an overview of the existing techniques, for further inquiry one can see the papers \cite{Wesolowski}\cite{Boneh2018}. We recall here that the proof consists in computing $\pi=h^{\floor{2^\tau/l}}$.


\subsubsection{Long division}
Because of the size of $\tau$, $2^25$ for real life usage, representing $\floor{2^\tau/l}$ can be hard. Thus Boneh et al. \cite{Boneh2018} proposed an algorithm to compute in $2\cdot\tau$ RSA group operations the proof by using the long division in base 2 where the proof is computed iteratively as described in Algorithm~\ref{alg:long_division}.

\begin{algorithm}[ht]
\SetAlgoLined
\KwResult{}
 $\pi=1$, $r=1$\;
 \For{$k \leftarrow 1$ to $k=\tau$}{
  $b\leftarrow \floor{2\cdot r/l}$\\
  $r\leftarrow 2\cdot r\ \Mod l$\\
  $\pi=\pi^2\cdot h^b$
 }
 \textbf{return} $\pi$
 \caption{Long division computation of the proof}\label{alg:long_division}
\end{algorithm}


\subsubsection{Parallel computation}
The idea of this acceleration, described by Boneh et al. \cite{Boneh2018} consists in choosing before evaluation a value $s$ and while evaluating the VDF challenge, storing $s$ specific exponentiations of $h$. Once we need to compute the proof, knowing these precomputations allows to run the computation on $s$ separate thread, reducing the proof complexity from $\mathcal{O}(T)$ to $\mathcal{O}(T/s)$. Typical values for $s$ would be 100.


\subsection{Quantum resistance}
Richard Feynman first talked about quantum computers outperforming classic ones in certain tasks in the 80s \cite{Feynman1982}. However the first real quantum algorithm threatening the cryptographic world is due to Shor \cite{Shor} presenting an efficient algorithm to integer factoring and finding discrete logarithm.

This algorithm requires $3\cdot\ceil{\log_2(N)}$ qbits to factorize a number $N$ \cite{Monz2016}. For example, factorizing a 2048 bits number as we recommend using for the VDF would require 6,144 qbits to run. As for 2019, the biggest quantum computer is Google's Sycamore \cite{Arute2019} which is still far from several thousands. We might still have some decades before this VDF construction becomes obsolete. However the research on quantum-secure VDF constructions is active. Some examples can be found in~\cite{Boneh2019, DeFeo, Buterin2018}.

%can be  link the difficulty $d_i(t)$ of a node $i$ to its reputation $r_i(t)$ by the relation 
%\begin{equation}
%d_i(t)=C\cdot r_it(t)    
%\end{equation}
%with $C(t)$ a global value in the network allowing to adapt the global throughput of the nodes to avoid congestion. This value should not vary regularly and be directly related with the sum of all the computational power $\sum \limits_{i\in\mathcal{N}} K_i(t)$.


%We have analyzed the number of tokens per address both in Bitcoin and in IOTA to get an estimation of its probability distribution. We noticed that, in both cases, the distribution is highly skewed, where the top 1\% of the addresses own the 90\% of the tokens. The way this reputation would be attributed is still to be defined but should not be based on the stake of the nodes because it would allocate too much power to the leading group of nodes. We rather envision metric based on the participation in the gossip protocol and its amount of issued transactions.



%\subsection{AIMD-based congestion control}
%The Additive Increase Multiplicative Decrease (AIMD) protocol \cite{Low2017} is a classical protocol used for congestion detection in TCP communications where a node starts by issuing packets with a small window size and icreases it by one each time it receives an ACK. Once one the transmission times out, the window is divided by two and the node restarts increasing it additively each time it receives an ACK. This method allows the node to avoid congestion by using a lower bandwith than available almost all the time but not smaller than the half.

%We envision applying a version of this protocol to DLT's protocols using the VDFs. The idea is to consider that each time a node $i$ sees its latest transaction validated in a very short time (around a few seconds), it can increase its thoughput $\lambda_i(t)$ by a fixed value $\lambda_{fix}$ and when it sees that a transaction takes a longer time, it simply divides $\lambda_i(t)$ by a factor 2.

%However a difficulty here is to map this with the VDF difficulty $d_i(t)$. As the time spent evaluating the VDF is inversely proportional to the difficulty, we can state a constant factor $k_i$ such as
%\begin{equation}
%\lambda_i(t)=k_i/\cdot d_i(t)    
%\end{equation}
%which depends on the hardware used by the node. Then if we consider at time $t+1$ that the node $i$ has a throughput 
% \begin{equation}
% \lambda_i(t+1)=\lambda_i(t)+\lambda_{fix}    
% \end{equation}
% then the difficulty should vary by 
% \begin{equation}
% d_i(t+1) = \frac{d_i(t)}{1+\lambda_{fix}/k_i}
% \end{equation}
% This can be tricky to compute as determining $k_i$ is something complicated without secure timestamping in the protocol \cite{Popov2017a}. Inversely, the division process is easier because of the proportionality between $\lambda_i(t)$ and $d_i(t)$.

==> simulation_backup.tex <==
\section{Simulation results}\label{sec:simulation}
In this section, we present the results derived from the C++ implementation of the protocol proposed in Section~\ref{sec:protocol}. We currently use the \texttt{NTL} library for multi-precision modular arithmetic~\cite{NTL}, but we plan to replace it with the \texttt{GMP} library which promises fast computation and verification time. Our simulator runs on a laptop using a i7-7820HQ CPU @ 2.90GHz processor.

Specifically, we simulate a single node computing the \emph{evaluation}, \emph{proof} and \emph{verification} tasks of the protocol on a random binary sequence $m$. Additionally, in Section~\ref{sec:comparison}, we give some insights of the communication overhead of the protocol on the network with a comparison with PoW.
We set the following parameters: the difficulty $\tau$ spans between $2^{20}$ and $2^{24}$ which leads to an evaluation time from a few seconds to a couple of minutes; as for the modulus, we use $\lambda\in\{1024, 2048, 3072\}$ bit length according to the discussion in Section~\ref{sec:rsa_length}. The hashing function chosen is SHA-256.
\begin{table}[ht]
\centering
%\tabcolsep=0.11cm
\small
\begin{tabular}{c|c}
    \textbf{Parameter} & \textbf{Value}\\
    \hline
    $k$ & $128$\\
    $\lambda$ & $\{1024, 2048, 3072\}$\\
    $\tau$ & $2^j, j\in[20,24]$\\
\end{tabular}
\caption{Simulation parameters used.}
\label{tab:simulation_parameters}
\end{table}


In Section~\ref{sec:protocol_eval} we will present the simulation results of the \textit{evaluation}, \textit{proof} and \textit{verification} steps, and in Section~\ref{sec:comparison} we will present an analysis of the potential spamming capabilities of different hardware when computing VDF or PoW.


\subsection{Protocol evaluation}\label{sec:protocol_eval}

\subsubsection{Evaluation time analysis}\label{sec:eval_time}
In Figure~\ref{fig:eval_cpp}, we evaluate the time needed solve the VDF challenge, i.e., to solve the sequential squarings of Eq.~\eqref{eq:eval}. The plot depicts the evaluation time (in \textit{s}) as a function of the difficulty $\tau$ of the challenge in a linear scale. The computing time grows linearly with the challenge, which allows a good predictability of the challenge timing for a node. In spite of the hardware variation, the maximum improvement factor is less than 30 between a common CPU and a specialized FPGA hardware.



\begin{figure}
\centering
\includegraphics[width=\linewidth]{images/eval.pdf}
\caption{Time needed to compute the VDF challenge for different modulus lengths.}
\label{fig:eval_cpp}
\end{figure}


\subsubsection{Proof time analysis}
In Figure~\ref{fig:proof_cpp}, one can find the time needed to compute the proof, i.e., the pair $\{l, \pi\}$ as a function of the difficulty $\tau$ of the challenge in a semi-logarithmic scale. We have to mention that the proof has to be computed by the same VDF solver right \emph{after} the solution of the VDF challenge (because it uses the output $y$). We can observe that in our implementation it takes roughly the same time as the evaluation. As proved by theory~\cite{Wesolowski}, the proof can be parallelized by a certain amount of threads. We discuss in Section~\ref{sec:proof_improve} some techniques aiming to speed up this part of the protocol.
\begin{figure}
\centering
\includegraphics[width=\linewidth]{images/proof.pdf}
\caption{Time needed to compute the VDF proof for different modulus lengths.}
\label{fig:proof_cpp}
\end{figure}

\subsubsection{Verification time analysis}
One of the fundamental requirements in our protocol design was to guarantee a low verification time (see Section~\ref{sec:introduction}). In Figure~\ref{fig:verif_cpp}, we depict the verification time (in \textit{ms}) as a function of the difficulty $\tau$ of the challenge in a semi-logarithmic scale. We note that the verification is in the range of 1 \textit{ms} (for 1024-bit length modulus) to 5 \textit{ms} (for 3072-bit length modulus). This result allows to process up to one thousand transactions per second. While this result is already promising and valuable, many improvements can be made from the engineering (e.g., GMP implementation) and algorithmic (e.g., precomputation, multi exponentiation optimization) side.

In Figure~\ref{fig:k_variation}, we plot the verification time as a function of the difficulty $\tau$ of the challenge in a semi-logarithmic scale in which we use different hash functions $H(m)$ with $k\in\{96, 128, 160\}$ and a modulus with bit length $\lambda=2048$. We observe that the verification time remains around a few milliseconds for larger security values, $\lambda=2048$ and $k=128$, which prevents the dilemma between performances and security.

Furthermore, it concurs with the  Result~\ref{th:verif_result}, the important property that the verification time only depends on the modulus bit-length $\lambda$ and on the security parameter $k$, and not on the difficulty $\tau$ is validated. Besides it also confirms the theoretical formula, as for $k=96$, the verification time is around 1.9\,ms, for $k=128$ the verification time is around 2.5ms and so on.

\begin{figure}
\centering
\includegraphics[width=\linewidth]{images/verif.pdf}
\caption{Time needed to compute the VDF proof for different modulus lengths.}
\label{fig:verif_cpp}
\end{figure}

\begin{figure}
\centering
\includegraphics[width=\linewidth]{images/k_variation.pdf}
\caption{Time needed to compute the VDF proof for different values of $k$ and $\lambda=2048$.}
\label{fig:k_variation}
\end{figure}

\subsection{Communication overhead}\label{sec:comparison}
As said earlier, PoW is used in the currently IOTA implementation as a rate control mechanism. In this subsection, we will show how VDF compares to PoW in the IOTA protocol in terms of communication overhead.

Specialized hardware (e.g., FPGAs) optimizes the computation on two levels. Firstly, it computes elementary operations such as RSA squaring faster than a general purpose CPU. Second, it allows some parallelization in the same chip. However, this ability depends on the kind of problem the hardware solves. We have seen from Result~\ref{th:sequential} that, unlike PoW, VDF is intrinsically sequential and cannot be parallelized. Therefore, an anti spam mechanism based on VDF is an efficient way to prevent specialized hardware to acquire a towering spamming power.

In Table~\ref{tab:pow_vs_vdf}, we show the performance in the computation of PoW and VDF of three different devices: (i) regular CPU used in general purpose computers, (ii) FPGA which are reconfigurable hardware circuits and (iii) ASIC, application-specific integrated circuit. For each device, the table shows the hashrate (or the number of squaring per second) and the speed up compared a regular CPU. We note that, due to the possibility of parallelization, the hashrate of PoW can be improved by several orders of magnitude. For example, experimental results show that a PoW-optimized ASIC can compute PoW $10^8$ times faster than CPU. Furthermore, as the PoW is unlimitedly parallelizable, a cluster of ASICs would even multiply this value where the VDF is a sequential work and thus cannot be sped up by resource pooling. On the other hand, VDF-optimized ASIC hardware is still a research project, and does not have an actual implementation at the time the paper is written. 

\begin{table}
    \centering
    \begin{tabular}{c|cc|cc}
        \multirow{2}{*}{\textbf{Hardware}} & \multicolumn{2}{c|}{\textbf{PoW}} & \multicolumn{2}{c}{\textbf{VDF}}\\
        & \multicolumn{2}{c|}{Hash/s} & \multicolumn{2}{c}{Squaring/s} \\
        \hline
        CPU & $10^4$ & $\times1$ & $10^6$ & $\times1$\\
        FPGA & $10^{10}$ & $\times10^6$ & $3\cdot10^7$ &  $\times30$\\
        ASIC & $10^{12}$ & $\times10^8$ & \multicolumn{2}{c}{\textit{n/a}}\\
    \end{tabular}
    \caption{Performance comparison between PoW and VDF.}
    \label{tab:pow_vs_vdf}
\end{table}

The ability to largely increase the hashing power by ASICs leads to the possibility to spam the network whereas the VDF prevents such a behaviour. We show in Figure~\ref{fig:comparison} (and we report the source values in Table~\ref{tab:spam_pow_vdf}) the potential spamming power by the three categories of devices we have just discussed in the previous paragraph. We take IOTA transactions as an example: in the current implementation, the mean transaction size is 1.6\,KB; when using our VDF-based protocol, the transactions require an overhead of 288 bytes when $\lambda=2048$ and $k=128$. The current PoW difficulty in the IOTA requires a regular CPU to work for 10 seconds on average. A single node using a FPGA has the ability to generate a throughput up to 1.3\,Gbps, making denial-of-service attacks extremely easy; it is impressive to see that, for the same hardware, VDF bounds the spamming capability to a few kbps. %Needless to talk about the ASIC's performances where a single node can break the network's capacity whereas the VDF still limits to a few hundreds kilobytes. These values show that the VDFs can really mitigate congestion and spamming in a network.

\begin{table}
    \centering
    \begin{tabular}{c|r@{\hspace{0.3em}}l|r@{\hspace{0.3em}}l}
        \textbf{Hardware} & \multicolumn{2}{c|}{\textbf{PoW}} & \multicolumn{2}{c}{\textbf{{VDF}}}\\
        \hline
%        CPU     & 1.4\,kbps                 & 1.9\,kbps\\
%        FPGA    & $1.3\cdot10^6$\,kbps      & 58\,kbps\\
%        ASIC    & $1.2\cdot10^{11}$\,kbps   & $1.9\cdot10^3$\,kbps\\
        CPU     & 1.4   & \,kbps    & 1.9 & \,kbps\\
        FPGA    & 1.3   & \,Gbps    & 58  & \,kbps\\
        ASIC    & 120   & \,Tbps    & \multicolumn{2}{c}{\textit{n/a}}\\
    \end{tabular}
    \caption{Spamming potential comparison between PoW and VDF.}
    \label{tab:spam_pow_vdf}
\end{table}


\begin{figure}
    \centering
    \includegraphics[width=\linewidth]{images/histo_pow_vs_vdf.png}
    \caption{Visual representation in $\log_{10}$ of the bandwidth usage for PoW and VDFs with different hardware.}
    \label{fig:comparison}
\end{figure}
